Dynamics with Simultaneous Dissipations to Fermionic and Bosonic Reservoirs

We introduce a non-phenomenological framework based on the influence functional method to incorporate simultaneous interactions of particles with fermionic and bosonic thermal reservoirs. In the slow-motion limit, the electronic friction kernel becomes Markovian, enabling an analytical expression for the friction coefficient. The framework is applied to a prototypical electrochemical system, where the metal electrode and solvent act as fermionic and bosonic reservoirs, respectively. We investigate quantum vibrational relaxation of hydrogen on metal surfaces, showing that dissipation to electron-hole pairs reduces the relaxation time. Additionally, in solvated proton discharge, electronic friction prolongs charge transfer by delaying proton transitions between potential wells. This study provides new insights into the interplay of solvent and electronic dissipation effects, with direct relevance to electrochemical processes and other systems involving multiple thermal reservoirs.

==> xx.tex <==




==> yy.tex <==



